Graph Representations for Higher-Order Logic and Theorem Proving

This paper presents the first use of graph neural networks (GNNs) for higher-order proof search and demonstrates that GNNs can improve upon state-of-the-art results in this domain. Interactive, higher-order theorem provers allow for the formalization of most mathematical theories and have been shown to pose a significant challenge for deep learning. Higher-order logic is highly expressive and, even though it is well-structured with a clearly defined grammar and semantics, there still remains no well-established method to convert formulas into graph-based representations. In this paper, we consider several graphical representations of higher-order logic and evaluate them against the HOList benchmark for higher-order theorem proving.

==> figures/tactic_success.tex <==


\begin{tikzpicture}
\begin{semilogyaxis}[
	ylabel=Success rate in \% (logscale),
	xtick=data,
% 	xlabel={Length of proofs},
    enlarge y limits={value=.05,upper},
	legend style={
	    at={(0.185,0.117)},
	    anchor=north,
	    legend columns=-1},
    bar width=.5mm,
    height=7cm, width=17cm,
    tickwidth=0pt,
    ybar,
    symbolic x coords={ANTS,ASMMESON,CHOOSE,CONJ,DISCH,DISJ1,DISJ2,EQ,MATCHMP,MESON,COMB,ONCEREWRITE,PUREONCEREWRITE,PUREREWRITE,POP,REFL,REWRITE,SIMP,SUBST},
    x tick label style={rotate=45,anchor=east},
]
\addplot[fill=yellow!50]
	coordinates {(ANTS,07.1) (ASMMESON,00.6) (CHOOSE,00.3) (CONJ,00.9) (DISCH,63.9) (DISJ1,24.2) (DISJ2,11.9) (EQ,00.6) (MATCHMP,05.3) (MESON,05.3) (COMB,03.4) (ONCEREWRITE,50.3) (PUREONCEREWRITE,31.9) (PUREREWRITE,001.0) (POP,45.5) (REFL,05.4) (REWRITE,34.5) (SIMP,31.8) (SUBST,00.4)};
\addplot[fill=blue!50]
	coordinates {(ANTS,01.6) (ASMMESON,01.0) (CHOOSE,00.6) (CONJ,00.9) (DISCH,64.7) (DISJ1,01.7) (DISJ2,00.4) (EQ,00.6) (MATCHMP,00.2) (MESON,05.8) (COMB,01.2) (ONCEREWRITE,87.8) (PUREONCEREWRITE,94.3) (PUREREWRITE,06.8) (POP,39.9) (REFL,01.0) (REWRITE,34.4) (SIMP,24.1) (SUBST,01.2)};
\addplot[fill=red!50]
    coordinates {(ANTS,03.0) (ASMMESON,01.0) (CHOOSE,00.8) (CONJ,01.0) (DISCH,78.2) (DISJ1,02.2) (DISJ2,00.7) (EQ,00.8) (MATCHMP,00.8) (MESON,02.1) (COMB,01.1) (ONCEREWRITE,90.1) (PUREONCEREWRITE,91.3) (PUREREWRITE,07.2) (POP,36.5) (REFL,00.3) (REWRITE,34.6) (SIMP,17.9) (SUBST,01.3)};
\addplot[fill=green!50]
    coordinates {(ANTS,17.0) (ASMMESON,01.0) (CHOOSE,00.5) (CONJ,02.7) (DISCH,62.3) (DISJ1,00.4) (DISJ2,00.4) (EQ,01.3) (MATCHMP,06.8) (MESON,03.3) (COMB,01.2) (ONCEREWRITE,89.1) (PUREONCEREWRITE,89.4) (PUREREWRITE,03.1) (POP,32.7) (REFL,00.2) (REWRITE,31.0) (SIMP,17.1) (SUBST,01.2)};
\legend{BoW, 0 hops, 2 hops, 4 hops}
\end{semilogyaxis}
\end{tikzpicture}



==> figures/wang_vs_ours.tex <==

\begin{tikzpicture}
\begin{scope}[every node/.style={font=\ttfamily}]
    \node (equalityapp) at (0,-.2) {a};
    \node (equalityapp2) at (-1,-.8) {a};
    \node (equalityconst) at (-1.5,-1.6) {c};
    \node (equalityname) at (-1,-2.4) {{$=$}};
    \node[color=orange] (equalitytype) at (-2,-2.4) {fun};
    \node[color=orange] (bool) at (-2.5,-4) {bool};
    \node[color=orange] (typeAtoBool) at (-2,-3.2) {fun};
    \node[color=orange] (typeA) at (-1,-4) {A};
    
    \node (lambda2) at (0.2,-1.6) {l};
    
    \node (variablex) at (0.2,-3.2) {v};
    \node (namex) at (.7,-4) {x};
\end{scope}

\begin{scope}[>={Stealth},
              every edge/.style={draw}]
    % \path [-] (root) edge (forallconstant);
    % \path [-,color=orange] (forallconstant) edge (foralltype);
    % \path [-,color=orange] (foralltype) edge (typeAtoBool);
    \path [-,color=orange] (typeAtoBool) edge (typeA);
    \path [-,color=orange] (typeAtoBool) edge (bool);
    % \path [-,color=orange] (foralltype) edge[bend right=30] (bool);
    % \path [-] (forallconstant) edge (forallname);
    % \path [-] (root) edge (equalityapp);
    \path [-] (equalityapp) edge (equalityapp2);
    \path [-] (equalityapp) edge (lambda2);
    \path [-] (equalityapp2) edge (lambda2);
    \path [-] (equalityapp2) edge (equalityconst);
    \path [-,color=orange] (equalityconst) edge (equalitytype);
    \path [-] (equalityconst) edge (equalityname);
    \path [-,color=orange] (equalitytype) edge (typeAtoBool);
    \path [-,color=orange] (equalitytype) edge[bend left=20] (typeA);
    \path [-] (variablex) edge (namex);
    \path [-,color=orange] (variablex) edge (typeA);
    \path [-] (lambda2) edge[bend left=10] (variablex);
    \path [-] (lambda2) edge[bend right=10] (variablex);
\end{scope}
\end{tikzpicture}
%
\qquad\qquad
%
\begin{tikzpicture}
\begin{scope}[every node/.style={font=\ttfamily}]
    \node (equality) at (0,0) {{$=$}};
    \node (lambda1) at (-1,-1) {lambda};
    \node (lambda2) at (1,-1) {lambda};
    \node (var1) at (-1,-2) {VAR};
    \node (var2) at (1,-2) {VAR};
    \node (phantom) at (1,-3) {\phantom{asdf}};
\end{scope}

\begin{scope}[>={Stealth},
              every edge/.style={draw}]
    \path [-] (equality) edge (lambda1);
    \path [-] (equality) edge (lambda2);
    \path [-] (lambda1) edge (var1);
    \path [-] (lambda2) edge (var2);
\end{scope}
\end{tikzpicture}

